Learning to Orient Surfaces by Self-supervised Spherical CNNs

Defining and reliably finding a canonical orientation for 3D surfaces is key to many Computer Vision and Robotics applications. This task is commonly addressed by handcrafted algorithms exploiting geometric cues deemed as distinctive and robust by the designer. Yet, one might conjecture that humans learn the notion of the inherent orientation of 3D objects from experience and that machines may do so alike. In this work, we show the feasibility of learning a robust canonical orientation for surfaces represented as point clouds. Based on the observation that the quintessential property of a canonical orientation is equivariance to 3D rotations, we propose to employ Spherical CNNs, a recently introduced machinery that can learn equivariant representations defined on the Special Orthogonal group SO(3). Specifically, spherical correlations compute feature maps whose elements define 3D rotations. Our method learns such feature maps from raw data by a self-supervised training procedure and robustly selects a rotation to transform the input point cloud into a learned canonical orientation. Thereby, we realize the first end-to-end learning approach to define and extract the canonical orientation of 3D shapes, which we aptly dub Compass. Experiments on several public datasets prove its effectiveness at orienting local surface patches as well as whole objects.

==> acks.tex <==
\section*{Acknowledgments}
We would like to thank Injenia srl and UTFPR for partly supporting this research work.


==> results/3DMatch/tabular.tex <==
\begin{table}[h]
%     \resizebox{0.7\columnwidth}{!}{
      \centering
       \setlength{\tabcolsep}{2.5mm}
      {
      \small 
      \caption{\label{tbl:3dmatch_rep} LRF repeatability on the \threedm{} dataset. Best result for each row in bold.}
      \begin{tabular}{lcccccc}
      \toprule
      \multicolumn{7}{c}{LRF Repeatability (\lrfrep{} $\uparrow$)}\\
      \hline
	  & SHOT \cite{tombari2010unique}
	  & FLARE \cite{petrelli2012repeatable} 
	  & TOLDI \cite{yang2017toldi}
	  & 3DSN \cite{gojcic2019perfect}
	  & \algoname{} (w/o aug)
	  & \algoname{} \\ 
	  \hline
	  Kitchen 	& 0.189 & \textbf{0.330} & 0.171 & 0.181 & 0.274 & 0.315\\
	  Home 1	& 0.251 & 0.354 & 0.243 & 0.236 & 0.370 & \textbf{0.397}\\
	  Home 2	& 0.226 & 0.339 & 0.213 & 0.214 & 0.353 & \textbf{0.365}\\ 
	  Hotel 1  	& 0.194 & \textbf{0.385} & 0.213 & 0.216 & 0.347 & 0.370\\ 
	  Hotel 2  	& 0.193 & \textbf{0.405} & 0.223 & 0.226 & 0.349 & 0.393\\ 
	  Hotel 3  	& 0.240 & 0.407 & 0.261 & 0.276 & 0.406 & \textbf{0.446}\\ 
	  Study		& 0.186 & 0.351 & 0.195 & 0.192 & 0.307 & \textbf{0.356}\\ 
	  Lab  		& 0.220 & 0.310 & 0.198 & 0.223 & 0.360 & \textbf{0.361}\\
	  \hline
	  Mean		& 0.212 & 0.360 & 0.215 & 0.220 & 0.346 & \textbf{0.375}\\
      \hline
      \end{tabular}
      }
%     }
    \vspace{-3mm}
 
\end{table}



==> results/3DMatch/tabular_rotated.tex <==
\begin{table}[H]
    % \resizebox{0.7\columnwidth}{!}{
      \centering
       \setlength{\tabcolsep}{2.5mm}
      {\small 
      \caption{\label{tbl:3dmatch_rep_rot} LRF repeatability of Compass on \threedm{} and \threedm{} rotated.}
      \begin{tabular}{lcc}
      \toprule
      \multicolumn{3}{c}{LRF Repeatability (\lrfrep{} $\uparrow$)}\\
      \hline
	  & \algoname{} (\threedm{} rotated)
	  & \algoname{} (\threedm{})\\ 
	  \hline
	  Kitchen 	& 0.312 & 0.315\\
	  Home 1	& 0.391 & 0.397\\
	  Home 2	& 0.359 & 0.365\\ 
	  Hotel 1  	& 0.361 & 0.370\\ 
	  Hotel 2  	& 0.383 & 0.393\\ 
	  Hotel 3  	& 0.447 & 0.446\\ 
	  Study		& 0.348 & 0.356\\ 
	  Lab  		& 0.355 & 0.361\\
	  \hline
	  Mean		& 0.369 & 0.375\\
      \hline
      \end{tabular}
      }
    % }
    \vspace{-3mm}
 
\end{table}



==> results/ETH/tabular.tex <==
\begin{table}[H]
    % \resizebox{\columnwidth}{!}{
      \centering
       \setlength{\tabcolsep}{1.5mm}
      {\small
      \caption{\label{tbl:eth_rep} LRF repeatability on the \eth{} dataset. Best result for each row in bold.}
      \begin{tabular}{lccccccc}
      \toprule
      \multicolumn{8}{c}{LRF Repeatability (\lrfrep{}  $\uparrow$)}\\
      \hline
	  & SHOT \cite{tombari2010unique} 
	  & FLARE \cite{petrelli2012repeatable} 
	  & TOLDI \cite{yang2017toldi}
	  & 3DSN \cite{gojcic2019perfect}
	  & \thead{\algoname{}\\(w/o aug)}
	  & \thead{\algoname{}}
	  & \thead{\algoname{}\\(adapted)}\\ 
	  \hline
	  Gazebo Summer				& 0.293 & \textbf{0.345} & 0.241 & 0.241 & 0.291 & 0.337 & 0.330\\
      Gazebo Winter         	& 0.266 & 0.268 & 0.170 & 0.196 & 0.286 & 0.292 & \textbf{0.303}\\ 
      Wood Autumn				& 0.253 & 0.210 & 0.157 & 0.174 & 0.304 & 0.288 & \textbf{0.307}\\
      Wood Summer       		& 0.279 & 0.236 & 0.171 & 0.198 & 0.329 & 0.314 & \textbf{0.329}\\
      \hline
      {Mean}                    & 0.273 & 0.264 & 0.185 & 0.202 & 0.303 & 0.308 & \textbf{0.317}\\
      \hline
      \end{tabular}
      }
    % }
  \vspace{-5mm}
  
\end{table}



==> results/ModelNet/tabular.tex <==
\begin{figure}[t]
	\centering
	\resizebox{\columnwidth}{!}{
	\setlength{\tabcolsep}{-5pt}
    \renewcommand{\arraystretch}{0}
	\begin{tabular}{cccccc}

		\includegraphics[width=.11\textwidth]{results/ModelNet/ours/17_41_0_src.png}&
		\includegraphics[width=.11\textwidth]{results/ModelNet/ours/17_41_1_src.png}&
		\includegraphics[width=.11\textwidth]{results/ModelNet/ours/17_41_2_src.png}&
		\includegraphics[width=.11\textwidth]{results/ModelNet/ours/26_17_0_src.png}&
		\includegraphics[width=.11\textwidth]{results/ModelNet/ours/26_17_1_src.png}&
		\includegraphics[width=.11\textwidth]{results/ModelNet/ours/26_17_2_src.png}\\
		
		\includegraphics[width=.11\textwidth]{results/ModelNet/ours/17_41_0_trg.png}&
		\includegraphics[width=.11\textwidth]{results/ModelNet/ours/17_41_1_trg.png}&
		\includegraphics[width=.11\textwidth]{results/ModelNet/ours/17_41_2_trg.png}&
		\includegraphics[width=.11\textwidth]{results/ModelNet/ours/26_17_0_trg.png}&
		\includegraphics[width=.11\textwidth]{results/ModelNet/ours/26_17_1_trg.png}&
		\includegraphics[width=.11\textwidth]{results/ModelNet/ours/26_17_2_trg.png}\\
		
% 		\includegraphics[width=.11\textwidth]{results/ModelNet/ours/30_28_0_src.png}&
% 		\includegraphics[width=.11\textwidth]{results/ModelNet/ours/30_28_1_src.png}&
% 		\includegraphics[width=.11\textwidth]{results/ModelNet/ours/30_28_2_src.png}&
% 		\includegraphics[width=.11\textwidth]{results/ModelNet/ours/37_11_0_src.png}&
% 		\includegraphics[width=.11\textwidth]{results/ModelNet/ours/37_11_1_src.png}&
% 		\includegraphics[width=.11\textwidth]{results/ModelNet/ours/37_11_2_src.png}&
	
		
		
% 		\includegraphics[width=.11\textwidth]{results/ModelNet/ours/30_28_0_trg.png}&
% 		\includegraphics[width=.11\textwidth]{results/ModelNet/ours/30_28_1_trg.png}&
% 		\includegraphics[width=.11\textwidth]{results/ModelNet/ours/30_28_2_trg.png}&
% 		\includegraphics[width=.11\textwidth]{results/ModelNet/ours/37_11_0_trg.png}&
% 		\includegraphics[width=.11\textwidth]{results/ModelNet/ours/37_11_1_trg.png}&
% 		\includegraphics[width=.11\textwidth]{results/ModelNet/ours/37_11_2_trg.png}&

		
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/17_41_0_src.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/17_41_1_src.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/17_41_2_src.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/0_11_0_src.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/0_11_1_src.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/0_11_2_src.png}\\
		
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/17_41_0_trg.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/17_41_1_trg.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/17_41_2_trg.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/0_11_0_trg.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/0_11_1_trg.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/0_11_2_trg.png}\\
		
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/26_17_0_src.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/26_17_1_src.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/26_17_2_src.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/30_28_0_src.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/30_28_1_src.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/30_28_2_src.png}\\
		
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/26_17_0_trg.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/26_17_1_trg.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/26_17_2_trg.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/30_28_0_trg.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/30_28_1_trg.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/30_28_2_trg.png}\\
		
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/37_11_0_src.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/37_11_1_src.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/37_11_2_src.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/8_3_0_src.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/8_3_1_src.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/8_3_2_src.png}\\
		
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/37_11_0_trg.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/37_11_1_trg.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/37_11_2_trg.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/8_3_0_trg.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/8_3_1_trg.png}&
% 		\includegraphics[width=.16\textwidth]{results/ModelNet/ours/8_3_2_trg.png}\\

	\end{tabular}
	}
	\caption{Qualitative results on the \modelnet{}  dataset. Top row: randomly rotated input cloud. Bottom row: cloud oriented by Compass.}
	\label{fig:qualitative_ModelNet}
	
\end{figure}

==> results/SV/tabular.tex <==
\begin{table}[H]
    % \resizebox{\columnwidth}{!}{
      \centering
       \setlength{\tabcolsep}{0.9mm}
      {\small
      \caption{\label{tbl:stanford_rep} LRF repeatability on the \stanford{} dataset. Best result for each row in bold.}
      \begin{tabular}{lcccccccc}
      \toprule
      \multicolumn{9}{c}{\lrf{} Repeatability (\lrfrep{} $\uparrow$)}\\
      \hline
	  & SHOT \cite{tombari2010unique}
	  & FLARE \cite{petrelli2012repeatable}
	  & TOLDI \cite{yang2017toldi} 
	  & 3DSN \cite{gojcic2019perfect}
  	  & GFrames \cite{melzi2019gframes}
  	  & \thead{\algoname{}\\(w/o aug)}
	  & \thead{\algoname{}}
	  & \thead{\algoname{}\\(adapted)}
	  \\ 
	  \hline
	  Armadillo		& 0.127 & 0.185 & 0.156  & 0.141 & 0.168 & 0.311 & 0.340 & \textbf{0.359}\\
      Buddha        & 0.134 & 0.194 & 0.202  & 0.192 & 0.181 & 0.295 & 0.312 & \textbf{0.344}\\ 
      Bunny			& 0.106 & 0.379 & 0.232  & 0.172 & 0.426 & 0.358 & 0.440 & \textbf{0.463}\\
      Dragon       	& 0.161 & 0.207 & 0.201  & 0.188 & 0.251 & 0.343 & 0.352 & \textbf{0.384}\\
      \hline
      {Mean}       	& 0.132 & 0.241 & 0.197  & 0.173 & 0.256 & 0.326 & 0.361 & \textbf{0.388}\\
      \hline
      \end{tabular}
      }
    % }
  \vspace{-3mm}
  
\end{table}



==> results/ShapeNET/table_comparison_training_modes.tex <==
\begin{figure}[htb]
	\centering
	\resizebox{0.9\columnwidth}{!}{
    \subfloat[Category-specific training]{
    	\setlength{\tabcolsep}{-2mm}
    	\renewcommand{\arraystretch}{2}
    	\begin{tabular}{ccc}
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/single_object_train/3c7e4628a9ea201bbf3143b1cb6076a_0_src.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/single_object_train/3c7e4628a9ea201bbf3143b1cb6076a_1_src.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/single_object_train/3c7e4628a9ea201bbf3143b1cb6076a_2_src.png}\\
    		
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/single_object_train/3c7e4628a9ea201bbf3143b1cb6076a_0_trg.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/single_object_train/3c7e4628a9ea201bbf3143b1cb6076a_1_trg.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/single_object_train/3c7e4628a9ea201bbf3143b1cb6076a_2_trg.png}\\
    		
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/single_object_train/1e6f06d182094d4ffebad4f49b26ec52_0_src.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/single_object_train/1e6f06d182094d4ffebad4f49b26ec52_1_src.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/single_object_train/1e6f06d182094d4ffebad4f49b26ec52_2_src.png}\\
    		
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/single_object_train/1e6f06d182094d4ffebad4f49b26ec52_0_trg.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/single_object_train/1e6f06d182094d4ffebad4f49b26ec52_1_trg.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/single_object_train/1e6f06d182094d4ffebad4f49b26ec52_2_trg.png}\\
    		    		
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/single_object_train/5ffcd5bc4f1548181c7f081cf615f39b_0_src.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/single_object_train/5ffcd5bc4f1548181c7f081cf615f39b_1_src.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/single_object_train/5ffcd5bc4f1548181c7f081cf615f39b_2_src.png}\\
    		
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/single_object_train/5ffcd5bc4f1548181c7f081cf615f39b_0_trg.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/single_object_train/5ffcd5bc4f1548181c7f081cf615f39b_1_trg.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/single_object_train/5ffcd5bc4f1548181c7f081cf615f39b_2_trg.png}\\
    	\end{tabular}
    }
    \subfloat[Category-agnostic training]{
        \setlength{\tabcolsep}{-2mm}
        \renewcommand{\arraystretch}{2}
        	\begin{tabular}{ccc}
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/multiple_objects_train/3c7e4628a9ea201bbf3143b1cb6076a_0_src.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/multiple_objects_train/3c7e4628a9ea201bbf3143b1cb6076a_1_src.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/multiple_objects_train/3c7e4628a9ea201bbf3143b1cb6076a_2_src.png}\\
    		
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/multiple_objects_train/3c7e4628a9ea201bbf3143b1cb6076a_0_trg.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/multiple_objects_train/3c7e4628a9ea201bbf3143b1cb6076a_1_trg.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/multiple_objects_train/3c7e4628a9ea201bbf3143b1cb6076a_2_trg.png}\\
    		
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/multiple_objects_train/1e6f06d182094d4ffebad4f49b26ec52_0_src.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/multiple_objects_train/1e6f06d182094d4ffebad4f49b26ec52_1_src.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/multiple_objects_train/1e6f06d182094d4ffebad4f49b26ec52_2_src.png}\\
    		
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/multiple_objects_train/1e6f06d182094d4ffebad4f49b26ec52_0_trg.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/multiple_objects_train/1e6f06d182094d4ffebad4f49b26ec52_1_trg.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/multiple_objects_train/1e6f06d182094d4ffebad4f49b26ec52_2_trg.png}\\
    		    		
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/multiple_objects_train/5ffcd5bc4f1548181c7f081cf615f39b_0_src.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/multiple_objects_train/5ffcd5bc4f1548181c7f081cf615f39b_1_src.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/multiple_objects_train/5ffcd5bc4f1548181c7f081cf615f39b_2_src.png}\\
    		
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/multiple_objects_train/5ffcd5bc4f1548181c7f081cf615f39b_0_trg.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/multiple_objects_train/5ffcd5bc4f1548181c7f081cf615f39b_1_trg.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/multiple_objects_train/5ffcd5bc4f1548181c7f081cf615f39b_2_trg.png}\\
    	\end{tabular}
    }
    
    \subfloat[Transfer learning]{
        \setlength{\tabcolsep}{-2mm}
        \renewcommand{\arraystretch}{2}
        	\begin{tabular}{ccc}
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/transfer_learning/3c7e4628a9ea201bbf3143b1cb6076a_0_src.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/transfer_learning/3c7e4628a9ea201bbf3143b1cb6076a_1_src.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/transfer_learning/3c7e4628a9ea201bbf3143b1cb6076a_2_src.png}\\
    		
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/transfer_learning/3c7e4628a9ea201bbf3143b1cb6076a_0_trg.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/transfer_learning/3c7e4628a9ea201bbf3143b1cb6076a_1_trg.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/transfer_learning/3c7e4628a9ea201bbf3143b1cb6076a_2_trg.png}\\
    		
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/transfer_learning/1e6f06d182094d4ffebad4f49b26ec52_0_src.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/transfer_learning/1e6f06d182094d4ffebad4f49b26ec52_1_src.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/transfer_learning/1e6f06d182094d4ffebad4f49b26ec52_2_src.png}\\
    		
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/transfer_learning/1e6f06d182094d4ffebad4f49b26ec52_0_trg.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/transfer_learning/1e6f06d182094d4ffebad4f49b26ec52_1_trg.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/transfer_learning/1e6f06d182094d4ffebad4f49b26ec52_2_trg.png}\\
    		    		
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/transfer_learning/5ffcd5bc4f1548181c7f081cf615f39b_0_src.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/transfer_learning/5ffcd5bc4f1548181c7f081cf615f39b_1_src.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/transfer_learning/5ffcd5bc4f1548181c7f081cf615f39b_2_src.png}\\
    		
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/transfer_learning/5ffcd5bc4f1548181c7f081cf615f39b_0_trg.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/transfer_learning/5ffcd5bc4f1548181c7f081cf615f39b_1_trg.png}&
    		\includegraphics[width=.13\textwidth]{results/ShapeNET/transfer_learning/5ffcd5bc4f1548181c7f081cf615f39b_2_trg.png}\\
    	\end{tabular}
    }
    }
	
	
% 	}
	\caption{Qualitative results on ShapeNet dataset under different training strategies. Clouds in yellow represent randomly rotated input clouds and the blue ones represent those oriented by \algoname{}. In (a), we present orientation results after training \algoname{} with examples belonging only to a  specific category from ShapeNet; in (b), the orientation results after training \algoname{} with a training set comprising \textit{airplanes}, \textit{chairs} and \textit{lamps} together; and, in (c) the orientation results from the model trained on the \modelnet{} dataset and tested on the ShapeNet dataset.}
	\label{fig:qualitative_model_shapenet}
	\vspace{-1mm}
\end{figure}

==> results/ShapeNET/table_shapenet_transfer.tex <==
% % \begin{wrapfigure}[13]{r}{.5\columnwidth}
% \begin{figure}[htb]
% 	\centering
% % 	\resizebox{0.7\columnwidth}{!}{
% 	\setlength{\tabcolsep}{-5pt}
% 	\begin{tabular}{cccccc}

% 		\includegraphics[width=.11\textwidth]{results/ShapeNET/TransferLearning/4a9d3ce54c09a2da696b74614952b2d0_0_src.png}&
% 		\includegraphics[width=.11\textwidth]{results/ShapeNET/TransferLearning/4a9d3ce54c09a2da696b74614952b2d0_1_src.png}&
% 		\includegraphics[width=.11\textwidth]{results/ShapeNET/TransferLearning/4a9d3ce54c09a2da696b74614952b2d0_2_src.png}&
		
% 		\includegraphics[width=.11\textwidth]{results/ShapeNET/TransferLearning/1a44dd6ee873d443da13974b3533fb59_0_src.png}&
% 		\includegraphics[width=.11\textwidth]{results/ShapeNET/TransferLearning/1a44dd6ee873d443da13974b3533fb59_1_src.png}&
% 		\includegraphics[width=.11\textwidth]{results/ShapeNET/TransferLearning/1a44dd6ee873d443da13974b3533fb59_2_src.png}\\
		
% 		\includegraphics[width=.11\textwidth]{results/ShapeNET/TransferLearning/4a9d3ce54c09a2da696b74614952b2d0_0_trg.png}&
% 		\includegraphics[width=.11\textwidth]{results/ShapeNET/TransferLearning/4a9d3ce54c09a2da696b74614952b2d0_1_trg.png}&
% 		\includegraphics[width=.11\textwidth]{results/ShapeNET/TransferLearning/4a9d3ce54c09a2da696b74614952b2d0_2_trg.png}&
		
% 		\includegraphics[width=.11\textwidth]{results/ShapeNET/TransferLearning/1a44dd6ee873d443da13974b3533fb59_0_trg.png}&
% 		\includegraphics[width=.11\textwidth]{results/ShapeNET/TransferLearning/1a44dd6ee873d443da13974b3533fb59_1_trg.png}&
% 		\includegraphics[width=.11\textwidth]{results/ShapeNET/TransferLearning/1a44dd6ee873d443da13974b3533fb59_2_trg.png}\\
% 	\end{tabular}
% % 	}
% 	\caption{Qualitative results on the \shapenet{} dataset of the model trained on the \modelnet{} dataset. Top row: randomly rotated input cloud. Bottom row: cloud oriented by Compass. The rightmost examples show a failure case.}
% 	\label{fig:qualitative_shapenet}
	
% \end{figure}

% \begin{wrapfigure}[13]{r}{.5\columnwidth}
\begin{figure}[htb]
	\centering
% 	\resizebox{0.7\columnwidth}{!}{
	\setlength{\tabcolsep}{-10pt}
	\begin{tabular}{ccccccccc}

		\includegraphics[width=.16\textwidth]{results/ShapeNET/TransferLearning/46d2373fa05a4876bc913a3935f0ae10_0_src.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/TransferLearning/46d2373fa05a4876bc913a3935f0ae10_1_src.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/TransferLearning/46d2373fa05a4876bc913a3935f0ae10_2_src.png}&
		
		\includegraphics[width=.16\textwidth]{results/ShapeNET/TransferLearning/4a9d3ce54c09a2da696b74614952b2d0_0_src.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/TransferLearning/4a9d3ce54c09a2da696b74614952b2d0_1_src.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/TransferLearning/4a9d3ce54c09a2da696b74614952b2d0_2_src.png}&
		
		\includegraphics[width=.16\textwidth]{results/ShapeNET/TransferLearning/1a44dd6ee873d443da13974b3533fb59_0_src.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/TransferLearning/1a44dd6ee873d443da13974b3533fb59_1_src.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/TransferLearning/1a44dd6ee873d443da13974b3533fb59_2_src.png}\\
		
		\includegraphics[width=.16\textwidth]{results/ShapeNET/TransferLearning/1e6f06d182094d4ffebad4f49b26ec52_0_src.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/TransferLearning/1e6f06d182094d4ffebad4f49b26ec52_1_src.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/TransferLearning/1e6f06d182094d4ffebad4f49b26ec52_2_src.png}\\
		
		
		\includegraphics[width=.16\textwidth]{results/ShapeNET/TransferLearning/46d2373fa05a4876bc913a3935f0ae10_0_trg.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/TransferLearning/46d2373fa05a4876bc913a3935f0ae10_1_trg.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/TransferLearning/46d2373fa05a4876bc913a3935f0ae10_2_trg.png}&
		
		\includegraphics[width=.16\textwidth]{results/ShapeNET/TransferLearning/4a9d3ce54c09a2da696b74614952b2d0_0_trg.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/TransferLearning/4a9d3ce54c09a2da696b74614952b2d0_1_trg.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/TransferLearning/4a9d3ce54c09a2da696b74614952b2d0_2_trg.png}&
		
		\includegraphics[width=.16\textwidth]{results/ShapeNET/TransferLearning/1a44dd6ee873d443da13974b3533fb59_0_trg.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/TransferLearning/1a44dd6ee873d443da13974b3533fb59_1_trg.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/TransferLearning/1a44dd6ee873d443da13974b3533fb59_2_trg.png}\\
		
		\includegraphics[width=.16\textwidth]{results/ShapeNET/TransferLearning/1e6f06d182094d4ffebad4f49b26ec52_0_trg.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/TransferLearning/1e6f06d182094d4ffebad4f49b26ec52_1_trg.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/TransferLearning/1e6f06d182094d4ffebad4f49b26ec52_2_trg.png}  \\
	\end{tabular}
% 	}
	\caption{Qualitative results on the \shapenet{} dataset of the model trained on the \modelnet{} dataset. Top row: randomly rotated input cloud. Bottom row: cloud oriented by Compass. The rightmost examples show a failure case.}
	\label{fig:qualitative_shapenet}
	
\end{figure}

==> results/ShapeNET/tabular.tex <==
\begin{figure}[t]
	\centering
	\resizebox{\columnwidth}{!}{
	\setlength{\tabcolsep}{0pt}
	\begin{tabular}{cccccc}

		\includegraphics[width=.16\textwidth]{results/ShapeNET/ours/1e6f06d182094d4ffebad4f49b26ec52_0_src.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/ours/1e6f06d182094d4ffebad4f49b26ec52_1_src.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/ours/1e6f06d182094d4ffebad4f49b26ec52_2_src.png}&
		
		\includegraphics[width=.16\textwidth]{results/ShapeNET/ours/247dd48e4b6c029e4b3c42e318f3affc_0_src.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/ours/247dd48e4b6c029e4b3c42e318f3affc_1_src.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/ours/247dd48e4b6c029e4b3c42e318f3affc_2_src.png}\\
		
		\includegraphics[width=.16\textwidth]{results/ShapeNET/ours/1e6f06d182094d4ffebad4f49b26ec52_0_trg.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/ours/1e6f06d182094d4ffebad4f49b26ec52_1_trg.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/ours/1e6f06d182094d4ffebad4f49b26ec52_2_trg.png}&
		
		\includegraphics[width=.16\textwidth]{results/ShapeNET/ours/247dd48e4b6c029e4b3c42e318f3affc_0_trg.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/ours/247dd48e4b6c029e4b3c42e318f3affc_1_trg.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/ours/247dd48e4b6c029e4b3c42e318f3affc_2_trg.png} \\
		
		\includegraphics[width=.16\textwidth]{results/ShapeNET/ours/4a9d3ce54c09a2da696b74614952b2d0_0_src.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/ours/4a9d3ce54c09a2da696b74614952b2d0_1_src.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/ours/4a9d3ce54c09a2da696b74614952b2d0_2_src.png}&
		
		\includegraphics[width=.16\textwidth]{results/ShapeNET/ours/6dfb7b5b4bd0d5f9febad4f49b26ec52_0_src.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/ours/6dfb7b5b4bd0d5f9febad4f49b26ec52_1_src.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/ours/6dfb7b5b4bd0d5f9febad4f49b26ec52_2_src.png}\\
		
		\includegraphics[width=.16\textwidth]{results/ShapeNET/ours/4a9d3ce54c09a2da696b74614952b2d0_0_trg.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/ours/4a9d3ce54c09a2da696b74614952b2d0_1_trg.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/ours/4a9d3ce54c09a2da696b74614952b2d0_2_trg.png}&
		
		\includegraphics[width=.16\textwidth]{results/ShapeNET/ours/6dfb7b5b4bd0d5f9febad4f49b26ec52_0_trg.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/ours/6dfb7b5b4bd0d5f9febad4f49b26ec52_1_trg.png}&
		\includegraphics[width=.16\textwidth]{results/ShapeNET/ours/6dfb7b5b4bd0d5f9febad4f49b26ec52_2_trg.png}\\

	\end{tabular}
	}
	\caption{Qualitative visualizations on the \shapenet{} dataset.}
	\label{fig:qualitative_shapenet}
	
\end{figure}

==> results/qualitative_LRF.tex <==
\begin{figure}[h]
	\centering
	\resizebox{\columnwidth}{!}{
    \renewcommand{\arraystretch}{0}
	\subfloat[Compass]{
	\begin{tabular}{cc}

		\includegraphics[width=.20\textwidth]{results/SV/qualitative/bunny_ours_src_rep.png}&
		\includegraphics[width=.20\textwidth]{results/SV/qualitative/bunny_ours_trg_rep.png}\\
		
		\includegraphics[width=.20\textwidth]{results/3DMatch/qualitative/home_ours_src_rep.png}&
		\includegraphics[width=.20\textwidth]{results/3DMatch/qualitative/home_ours_trg_rep.png}\\
	\end{tabular}
	}
	\subfloat[FLARE]{
    \begin{tabular}{cc}

		\includegraphics[width=.20\textwidth]{results/SV/qualitative/bunny_flare_src_rep.png}&
		\includegraphics[width=.20\textwidth]{results/SV/qualitative/bunny_flare_trg_rep.png}
		\\
		
		\includegraphics[width=.20\textwidth]{results/3DMatch/qualitative/home_flare_src_rep.png}&
		\includegraphics[width=.20\textwidth]{results/3DMatch/qualitative/home_flare_trg_rep.png}\\
	\end{tabular}
	}
	}
	\caption{Visualization of repeatability at corresponding points of two fragments, with repeatable LRFs in green, non-repeatable ones in red and non-overlapping areas in gray. First row:  a pair of fragments from Stanford Views, second  row: a pair of fragments from 3DMatch.  (a) and (b): results yielded  by  Compass and FLARE, respectively.}
	%\caption{Qualitative visualizations on the Stanford Views (first row) and 3DMatch (second row). For each dataset, we get a pair of fragments and estimate if each point is repeatable or not. Green values represent repeatable LRFs and red values non-repeatable. The gray area represents non-overlapped points, and consequently, with no estimated values.}
	\label{fig:qualitative_repeatability}
	
\end{figure}


\begin{figure}[h]
	\centering
	\resizebox{\columnwidth}{!}{
    \renewcommand{\arraystretch}{0}
	\subfloat[Compass]{
    	\begin{tabular}{cc}
    
    		\includegraphics[width=.20\textwidth]{results/SV/qualitative/bunny_ours_src_theta.png}&
    		\includegraphics[width=.20\textwidth]{results/SV/qualitative/bunny_ours_trg_theta.png}
    		\\
    		
    		\includegraphics[width=.20\textwidth]{results/3DMatch/qualitative/home_ours_src_theta.png}&
    		\includegraphics[width=.20\textwidth]{results/3DMatch/qualitative/home_ours_trg_theta.png}\\
    	\end{tabular}
    	}
    	\subfloat[FLARE]{
    	\begin{tabular}{cc}
    
    		\includegraphics[width=.20\textwidth]{results/SV/qualitative/bunny_flare_src_theta.png}&
    		\includegraphics[width=.20\textwidth]{results/SV/qualitative/bunny_flare_trg_theta.png}
    		\\
    		
    		\includegraphics[width=.20\textwidth]{results/3DMatch/qualitative/home_flare_src_theta.png}&
    		\includegraphics[width=.20\textwidth]{results/3DMatch/qualitative/home_flare_trg_theta.png}\\
    	\end{tabular}
    	}
	}
	\caption{Visualization of the angular error between the LRFs estimated at corresponding points of two fragments, with lower errors in blue, higher errors in red and non-overlapping areas in gray. First row:  a pair of fragments from Stanford Views. Second  row: a pair of fragments from 3DMatch.  (a) and (b): results yielded by Compass and FLARE, respectively.}
	\label{fig:qualitative_theta}
\end{figure}


